Holographic solutions from 5D $SO(2)\times ISO(3)$ $N=4$ gauged supergravity

We study various types of holographic solutions from five-dimensional $N=4$ gauged supergravity coupled to three vector multiplets with $SO(2)\times ISO(3)$ gauge group. This gauged supergravity can be obtained from the maximal gauged supergravity in seven dimensions on a Riemann surface. For a negatively curved Riemann surface $H^2$, the resulting five-dimensional gauged supergravity admits a supersymmetric $N=4$ $AdS_5$ critical point. This $AdS_5$ vacuum is dual to an $N=2$ superconformal field theory (SCFT) arising from M5-branes wrapped on $H^2$. We study holographic RG flows between this SCFT and $N=2$ non-conformal phases by deformations involving relevant, marginal and irrelevant operators. Solutions describing conformal interfaces between these non-conformal phases and singular boundaries are also given. We finally study a number of supersymmetric $AdS_5$ black string and black hole solutions holographically dual to RG flows across dimensions from the $N=2$ SCFT to two-dimensional SCFTs and superconformal quantum mechanics in the IR. A number of solutions describing black strings and black holes in asymptotically domain wall space-time are also found. All of the solutions can be uplifted to M-theory by a consistent truncation on $H^2\times S^4$.

==> ref_list.tex <==
\bibitem{maldacena} J. M. Maldacena, ``The large $N$ limit of superconformal field theories and supergravity'', Adv. Theor. Math. Phys. \textbf{2} (1998) 231-252, arXiv: hep-th/9711200.
\bibitem{Gubser_AdS_CFT} S. S. Gubser, I. R. Klebanov and A. M. Polyakov, ``'', Phys. Lett. \textbf{B428} (1998) 105-114, arXiv: hep-th/9802.109.
\bibitem{Witten_AdS_CFT} E. Witten, ``Anti De Sitter Space and holography'', Adv. Theor. Math. Phys. \textbf{2} (1998) 253-291, arXiv: 9802150.
\bibitem{ISO3_5D_N4_gauntlett} K. C. M. Cheung, J. P. Gauntlett, C. Rosen, ``Consistent KK truncations for M5-branes wrapped on Riemann surfaces'', Class. Quant. Grav. \textbf{36} (2019) 22, 225003 , arXiv: 1906.08900.
\bibitem{M-theory_on_S4_1} H. Nastase, D. Vaman, and P. van Nieuwenhuizen, ``Consistent nonlinear KK
reduction of 11-d supergravity on $AdS_7\times S^4$ and selfduality in odd dimensions'', Phys. Lett. \textbf{B469} (1999) 96–102, arXiv: hep-th/9905075.
\bibitem{M-theory_on_S4_2} H. Nastase, D. Vaman, and P. van Nieuwenhuizen, ``Consistency of the $AdS_7\times S^4$ reduction and the origin of selfduality in odd dimensions'', Nucl. Phys. \textbf{B581} (2000) 179–239, arXiv: hep-th/9911238.
\bibitem{Malek_AdS5_N4_embed} E. Malek and V. V. Camell, ``Consistent truncations around half-maximal $AdS_5$ vacua of 11-dimensional supergravity'', Class. Quant. Grav. \textbf{39} (2022) 7, 075026, arXiv: 2012.15601.
\bibitem{GPPZ} L. Girardello, M. Petrini, M. Porrati, and A. Zaffaroni, ``Novel local CFT and exact
results on perturbations of $N=4$ super Yang Mills from AdS dynamics, JHEP 12 (1998) \textbf{022}, arXiv: hep-th/9810126.
\bibitem{FGPP} D. Z. Freedman, S. S. Gubser, K. Pilch, and N. P. Warner, ``Renormalization group
flows from holography supersymmetry and a c theorem'', Adv. Theor. Math. Phys. \textbf{3} (1999) 363–417, arXiv: hep-th/9904017.
\bibitem{KW_5Dflow} A. Khavaev and N. P. Warner, ``A Class of $N=1$ Supersymmetric RG Flows from Five-dimensional $N=8$ Supergravity'', Phys. Lett. \textbf{B495} (2000) 215-222, arXiv: hep-th/0009159.
\bibitem{N2_IIB_flow} K. Pilch and N. P. Warner, ``$N=2$ Supersymmetric RG Flows and the IIB Dilaton'', Nucl. Phys. \textbf{B594} (2001) 209-228, arXiv: hep-th/0004063.
\bibitem{AdS_RG_flow} N. Evans and M. Petrini, ``AdS RG-Flow and the Super-Yang-Mills Cascade'', Nucl. Phys. \textbf{B592} (2001) 129-142, arXiv: hep-th/0006048.
\bibitem{N1_SYM_fixed_point} K. Behrndt, ``Domain walls of $D=5$ supergravity and fixed points of $N=1$ Super Yang Mills'', Nucl. Phys. \textbf{B573} (2000) 127-148, arXiv: hep-th/9907070.
\bibitem{5D_N4_flow_Davide} N. Bobev, D. Cassani and H. Triendl, ``Holographic RG Flows for Four-dimensional $N=2$ SCFTs'', JHEP 06(2018)\textbf{086}, arXiv: 1804.03276.
\bibitem{5D_N4_flow} H. L. Dao and P. Karndumri, ``Holographic RG flows and $AdS_5$ black strings from 5D half-maximal gauged supergravity'', arXiv: 1811.01608.
\bibitem{Davide_5D_DW} D. Cassani, G. Dall’Agata and A. F. Faedo, ``BPS domain walls in $N=4$ supergravity and dual flows'', JHEP 03 (2013) \textbf{007}, arXiv: 1210.8125.
\bibitem{5D_N2_DW1} A. Ceresole, G. Dall'Agata, R. Kollosh and A. Van Proeyen, ``Hypermultiplets, domain walls and supersymmetric attractors'' Phys. Rev. \textbf{D64} (2001) 104006, arXiv: hep-th/0104056.
\bibitem{Calos_5D_N4_flow} A. F. Faedo, C. Nunez and C. Rosen, ``Consistent truncations of supergravity and $\frac{1}{2}$-BPS RG flows in $4d$ SCFTs'', JHEP 03 (2020) \textbf{080}, arXiv: 1912.13516.
\bibitem{5D_flowII} P. Karndumri, ``$AdS_5$ vacua and holographic RG flows from 5D $N=4$ gauged supergravity'', Eur. Phys. J. \textbf{C83} (2023) 164, arXiv: 2209.05270.
\bibitem{Bak_Janus} D. Bak, M. Gutperle and S. Hirano, ``A Dilatonic Deformation of $AdS_5$ and its Field Theory Dual'', JHEP 05 (2003) \textbf{072}, arXiv: hep-th/0304129.
\bibitem{5D_Janus_CK} A. Clark and A. Karch, ``Super Janus'', JHEP 10 (2005) \textbf{094}, arXiv: hep-th/0506265.
\bibitem{Freedman_Janus} A. B. Clark, D. Z. Freedman, A. Karch and M. Schnabl, ``Dual of the Janus solution: An interface conformal field theory'', Phys. Rev. \textbf{D71} (2005)
066003, arXiv: hep-th/0407073.
\bibitem{DHoker_Janus} E. D' Hoker, J. Estes and M. Gutperle, ``Interface Yang-Mills, supersymmetry, and Janus'', Nucl. Phys. \textbf{B753} (2006) 16, arXiv: hep-th/0603013.
\bibitem{5D_Janus_Suh} M. W. Suh, ``Supersymmetric Janus solutions in five and ten dimensions'', JHEP 09 (2011)
\textbf{064}, arXiv: 1107.2796.
\bibitem{Bobev_5D_Janus1} N. Bobev, F. F. Gautason, K. Pilch, M. Suh, J. van Muiden, ``Janus and J-fold Solutions from Sasaki-Einstein Manifolds'', Phys. Rev. \textbf{D100} (2019) 081901, arXiv: 1907.11132.
\bibitem{Bobev_5D_Janus2} N. Bobev, F. F. Gautason, K. Pilch, M. Suh, J. van Muiden, ``Holographic Interfaces in $N=4$ SYM: Janus and J-folds'', JHEP 05 (2020) \textbf{134}, arXiv: 2003.09154.
\bibitem{5D_N4_Janus} P. Karndumri, ``Janus and RG-flow interfaces from $5D$ $N=4$ gauged supergravity'', Phys. Rev. \textbf{D111} (2025) 12, 126020, arXiv: 2503.06704.
\bibitem{Witten_twist} E. Witten, ``Topological Quantum Field Theory'', Commun. Math. Phys. 117 (1988) \textbf{353}.
\bibitem{MN_nogo} J. M. Maldacena and C. Nunez, ``Supergravity description of field theories on curved manifolds and a no go theorem'', Int. J. Mod. Phys. \textbf{A16} (2001) 822-855, arXiv: hep-th/0007018.
\bibitem{black_string_Klemm1} D. Klemm and W. A. Sabra, ``Supersymmetry of black strings in $d = 5$ gauged supergravities'', Phys. Rev. \textbf{D62} (2000) 024003, arXiv: hep-th/0001131.
\bibitem{black_string_Klemm2} S. L. Cacciatori, D. Klemm and W. A. Sabra, ``Supersymmetric domain walls and strings in $d=5$ gauged supergravity coupled to vector multiplets'', JHEP 03 (2003) \textbf{023}, arXiv: hep-th/0302218.
\bibitem{black_string_Klemm3} A. Bernamonti, M. M. Caldarelli, D. Klemm, R. Olea, C. Sieg and E. Zorzan, ``Black strings in $AdS_5$'', JHEP 01 (2008) \textbf{061}, arXiv: 0708.2402.
\bibitem{BB} F. Benini and N. Bobev, ``Two-dimensional SCFTs from wrapped branes and
c-extremization'', JHEP 06 (2013) \textbf{005}, arXiv: 1302.4451.
\bibitem{Wraped_D3} P. Karndumri and E. O Colgain, ``3D Supergravity from wrapped D3-branes'', JHEP 10 (2013) \textbf{094}, arXiv: 1307.2086.
\bibitem{3D_CFT_from_LS_point} N. Bobev, K. Pilch, and O. Vasilakis, ``$(0,2)$ SCFTs from the Leigh-Strassler fixed point'', JHEP 06 (2014) \textbf{094}, arXiv:1403.7131.
\bibitem{BBC} F. Benini, N. Bobev and P. M. Crichigno, ``Two-dimensional SCFTs from D3-branes'', JHEP 07 (2016) \textbf{020}, arXiv: 1511.09462.
\bibitem{black_string_Klemm4} D. Klemm, N. Petri and M. Rabbiosi, ``Black string first order flow in $N=2$, $d = 5$ abelian gauged supergravity'', JHEP 01 (2017) \textbf{106}, arXiv: 1610.07367.
\bibitem{flow_acrossD_bobev} N. Bobev and P. M. Crichigno, ``Universal RG Flows Across Dimensions and Holography'', JHEP 12 (2017) 065, arXiv: 1708.05052.
\bibitem{black_string_Klemm5} M. Azzola, D. Klemm and M. Rabbiosi, ``$AdS_5$ black strings in the stu model of FI-gauged $N=2$ supergravity'', JHEP 10 (2018) \textbf{080}, arXiv: 1803.03570.
\bibitem{flow_across_Betti} A. Amariti and C. Toldo, ``Betti multiplets, flows across dimensions and c-extremization'', JHEP 07 (2017) \textbf{040}, arXiv: 1610.08858.
\bibitem{5D_N4_flow} H. L. Dao and P. Karndumri, ``Holographic RG flows and $AdS_5$ black strings from 5D half-maximal gauged supergravity'', Eur. Phys. J. \textbf{C79} (2019) 137, arXiv: 1811.01608.
\bibitem{5D_N4_flow1} H. L. Dao and P. Karndumri, ``Supersymmetric  black holes and strings from 5D  gauged supergravity'', Eur. Phys. J. \textbf{C79} (2019) 247, arXiv: 1812.10122.
C. Couzens, N. T. Macpherson and A. Passias, $N=(2, 2)$ $AdS_3$ from D3-branes wrapped
on Riemann surfaces, JHEP 02 (2022) \textbf{189}, arXiv: 2107.13562.
\bibitem{5D_N4_black_stringII} P. Karndumri, ``New supersymmetric $AdS_5$ black strings from 5D $N=4$ gauged supergravity'', Eur. Phys. J. \textbf{C83} (2023) 432, arXiv: 2211.07456.
\bibitem{N4_gauged_SUGRA} J. Schon and M. Weidner, ``Gauged $N=4$ supergravities'', JHEP 05 (2006) \textbf{034}, arXiv: hep-th/0602024.
\bibitem{5D_N4_Dallagata} G. Dall’Agata, C. Herrmann, and M. Zagermann, ``General matter coupled $N=4$ gauged supergravity in five-dimensions'', Nucl. Phys. \textbf{B612} (2001) 123–150, arXiv: hep-th/0103106.
\bibitem{Gubser_Sing} Steven S. Gubser, ``Curvature singularities: the good, the bad and the naked,” Adv. Theor. Math. Phys. \textbf{4} (2000), 679-745, arXiv: hep-th/0002160.
\bibitem{BCFT_Gutperle} M/ Gutperle and J. Samani, ``Holographic RG-flows and Boundary CFTs'', Phys. Rev. \textbf{D86} (2012) 106007, arXiv: 1207.7325.

\bibitem{Romans_5DN4} L. J. Romans, ``Gauged $N=4$ supergravities in five dimensions and their magnetovac backgrounds'', Nucl. Phys. \textbf{B267} (1986) 433,
\bibitem{Gauntlett_pure_5DN4_from_11D} J. P. Gauntlett and O. Varela, ``$D=5$ $SU(2)\times U(1)$ gauged supergravity from $D=11$ supergravity'', JHEP 02 (2008) \textbf{083}, arXiv: 0712.3560.
\bibitem{AdS5_BH_Romans} H. Nieder and Y. Oz, ``Supergravity and D-branes Wrapping Supersymmetric 3-Cycles'', JHEP 03 (2001) \textbf{008}, arXiv: hep-th/0011288.
''




\bibitem{line_defects_5DN4_Nicolo} F. Faedo, N. Petri and A. Segati, ``Defects in 4d SCFTs from supergravity and holographic renormalization'', JHEP 05 (2025) \textbf{070}, arXiv: 2501.17923.
\bibitem{Gauntlett_D3_spindle} P. Ferrero, J. P. Gauntlett, J. M. Perez Ipina, D. Martelli and J. Sparks, ``D3-Branes Wrapped on a Spindle'', Phys. Rev. Lett. \textbf{126} (2021) 111601, arXiv: 2011.10579.
\bibitem{Minwoo_D3_spindle} M. Suh, ``D3-branes and M5-branes wrapped on a topological disc'', JHEP 03 (2022) \textbf{043}, arXiv: 2108.01105.






